Dynamical feasibility of (3) Juno as a parent body of the H chondrites

We test the hypothesis that (3) Juno is a parent body of the H chondrites with dynamical modeling of an asteroid-family-forming impact and comparison to current observational data. Using a dynamical model that includes the Yarkovsky force on a simulated Juno family and a simplified cosmic ray exposure age model we examine the expected distribution of Juno family members in both the main belt and near-Earth orbits over 300 Myrs and the cosmic ray exposure distribution for fragments exiting the main belt via the 3:1J, 5:2J, and 8:3J mean motion resonances. We find that the smallest modeled ($D<$10 m) family members of (3) Juno cannot be directly responsible for the observed H chondrite flux and that the breakup of larger family members creates an CRE distribution that resembles the measured H chondrite CRE distribution but is still unable to adequately explain the significant number of H chondrites with CRE ages of 6-8 Myrs. A similar model was performed for the asteroid (6) Hebe, another parent body candidate, and produced a CRE age distribution that is inconsistent with the measured H chondrite CRE ages. We also find from our dynamical models that we can expect $<$7 km-scale Juno family members in near-Earth orbits in the present day, consistent with the recent discovery of the shock-darkened H chondrite-like asteroid (52768) 1998 OR$_{2}$.

==> old_text.tex <==
\textcolor{red}{From the Methods}
In the stead of a full YORP force calculation reliant on each asteroid's thermal inertia and rotation state, we use the radial drift rates for main belt asteroids provided in Figure 2 of \cite{2006AREPS..34..157B} and scale these values by the inverse square of each asteroid's heliocentric distance in every timestep. The resulting acceleration is added to the particle's acceleration vector via the following equations:
\begin{equation}
    a_x = \frac{-v_x}{2a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
\begin{equation}
     a_y = \frac{-v_y}{2a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
\begin{equation}
     a_z = \frac{-v_z}{2a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
and the corresponding velocity is added to each test particles velocity by a similar set of equations:
\begin{equation}
    a_x = \frac{x}{a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
\begin{equation}
     a_y = \frac{y}{a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
\begin{equation}
     a_z = \frac{z}{a}c(\frac{a_{Juno}^{2}}{a^2})
\end{equation}
In these equations $c$ represents the AU/yr drift rate of the test particles, which are chosen based on Figure 2a in \cite{2006AREPS..34..157B} for the diameter of each test particle size assuming a surface conductivity of $\kappa$=0.001 W m$^{-1}$.

To determine the significance that the Yarkovsky effect has on the flux of test particles reaching major resonances as well on the impact that family location has on family dynamics we ran three control tests. A table of initial parameters for the control cases is given in Table \ref{tab:init_parameters}. These control tests have the drift rate value $c$ set to 0 and are initiated at perihelion, mid-helion, and aphelion. No significant differences between the control datasets were identified. 

For the experimental tests four drift rates were chosen that correspond to three orders of magnitude in particle diameter, from one meter up to one kilometer. These sizes and drift rates are given in Table \ref{tab:exp_parameters}. For each drift rate 10 families of 100 test particles were generated, with 5 families given radially outward drifts (i.e. test particle rotation axes is parallel to orbital angular momentum vector) or radially inward (i.e. rotation axis is anti-parallel to orbital angular momentum). Each family was integrated for 300 Myr to understand behavior over the estimated age of the Juno family \citep{2019AJ....158..213N}.

\begin{table*}[]
    \centering
    \begin{tabular}{c |c| c| c| c }
        Julian Date & Initial Heliocentric Distance (au) & Total Number of Test\\
        Particles & Time Step & Integration Time\\
        \hline
         2459241.5 & 3.354 & 600 & 0.1 & 300 Myr \\
         2458778.5 & 2.668 & 600 & 0.1 & 300 Myr \\
         2458446.5 & 1.983 & 1000 & 0.1 & 300 Myr \\
    \end{tabular}
    \caption{Table of input parameters for control Rebound simulations. An example binary initialization file is available for download. }
    \label{tab:init_parameters}
\end{table*}
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
        Particle Diameter & Drift Rate (au/yr)  \\
        \hline
        1m & 1$0^{-8}$ \\
        10m & 2$\times10^{-9}$ \\ 
        100m & 7$\times10^{-10}$ \\
        1km & 8$\times10^{-11}$ \\
    \end{tabular}
    \caption{Table of initial parameters for experimental Rebound simulations. An example binary initialization file is available for download. }
    \label{tab:exp_parameters}
\end{table}

\textcolor{red}{From the Results}
The simulation results for the one meter diameter particles, which have the highest drift rates, are shown in Figures \ref{fig:a_e_t} and \ref{fig:particle_history}. The proximity of Juno to the weak 8:3 resonance with Jupiter allows the small one-meter particles to reach this resonance within just a few million years of family formation but only one-kilometer particles are actually scattered out of the resonance, due to the residence time required for scattering \citep{1997Sci...277..197G}. By far the most dominant scattering source of the test particles is the 3:1 mean motion resonance, which the one meter particles reach between 6-9 Myrs. No test particle drifting radially inward is able to successfully cross this resonance without scattering. The particles drifting radially outwards have a much longer time to completely scatter, with some particles making it all the way to the 2:1 mean motion resonance with Jupiter before finally being scattered around 80 Myrs. These particles also see a downward trend in eccentricity, bounded by interactions with Jupiter, once they have passed the 5:2 MMR. 

Once particles have passed the 5:2 MMR there is a continuum of particles that are scattered by Jupiter interactions (Fig. \ref{fig:particle_history}). This stands in sharp contrast to the large number of clustered scattering events between 5 and 15 MYrs, in which the majority of test particles are scattered. This would suggest that a large influx of the smallest Juno family members into near-Earth orbits $\sim$10 Myrs after the family forming event would then be followed by a relative trickle from particles evected by the more distant and less effective 5:2 resonance. 

As the drift rate decreases and the modeled particle size increases the number of particles reaching the removal criteria steadily decreases. Of the 1000 test particles in each simulation, 100\% of the 1 m particles, 99.8\% of 10 m, 70.6\% of 100 m, and 23.3\% of 1 km particles reach interactions with Mars and/or Jupiter. The one-kilometer particles nearly resemble the control groups (Figure \ref{fig:scatter_props}) and the Juno family members described in \cite{1995Icar..116..291Z}.  

\begin{table}[]
    \centering
    \begin{tabular}{c | c | c | c }
         Particle Diameter &   50\%   & 75\%  & 99\% \\
         \hline
         1 m & 13.3 &  15.7 & 59.9  \\
         10 m & 58.6 & 71.4 & 137.5 \\
         
    \end{tabular}
    \caption{Times to reach 50, 75, and 99\% scattering efficiencies for 1 m and 10 m  test particle effective sizes, which were the only particle populations to be completely scattered within the 300 Myr simulation. All times are give in Myrs.}
    \label{tab:scattering_timescales}
\end{table}

By far the most significant sources of scattering of Juno family members between 1 and 100 meters are the J3:1 and J5:2 resonances (c.f. Figures \ref{fig:scatter_props} and \ref{fig:histograms}). Table \ref{tab:scattering_timescales} details the timescales over which different percentages of the initial family members are effectively scattered via interactions with Mars and Jupiter, largely via the J3:1 and 5:2. The small particles reaching these resonances are preferentially removed via the inner Mars-crossing boundary condition and have previously established probabilities for entering Earth-crossing orbits \citep{1997Sci...277..197G,morbidelli2002origin}. Even with such a large percentage of particles smaller than 100 meters scattering, the efficiency of these particles entering Earth-crossing orbits is just 0.7\%, and of those 2$\time$10$^{-3}$ over the 2.2 Myr average lifetime in those orbits. 

For the larger Juno family members in the $\sim$1 km size range, the prolonged residency in the J8:3 resonance shows quite strongly in the parameters just prior to scattering (Figure \ref{fig:scatter_props}. With a much slower drift rate in the simulation the larger test particles see a nearly uniform scattering from this resonance over the duration of the simulation (Figure \ref{fig:histograms}. 

To validate this estimate we ran a second size independent simulation of particles in the 3:1 and 5:2 resonances more closely using the IAS15 integrator within the REBOUND code \cite{rein2015ias15}, which can resolve close planetary encounters with an adaptive timestep. We found that a similar number of particles collided with the Sun (\textcolor{red}{$\sim$72\%}), ended up in orbits outside of Saturn (\textcolor{red}{$\sim$27\%}), and entered Earth-crossing orbits (\textcolor{red}{$\sim$1\%}) as detailed in \cite{1997Sci...277..197G}.

\textcolor{red}{From the Discussion}
The models show that the 1 - 100 meter objects created by a Juno family impact should have all been susceptible to the 3:1 and 5:2 resonances and effectively diffused in 300 Myr. Juno family members 1 km or larger have not reached the 3:1 or 5:2 resonance by the end of the same time period, Assuming that the shock degassing and CRE ages are representative of the formation of the Juno family and the actual time spent susceptible to cosmic rays we find that H chondrites cannot be directly traced to Juno. Even the test particles approximating 1 m size test particles would still take between 10-12 Myr to arrive at the Earth, assuming the probabilities given in \cite{morbidelli2002origin}.

 Within these models we make several reasonable, albeit simple, assumptions regarding the formation and evolution of the Juno family. As previously described in Section \ref{sec:Methods} we use Yarkovsky drift rates associated with a surface conductivity of $\kappa$ = 0.001 W m$^{-1}$, taken from \cite{2006AREPS..34..157B}. Particles with similar $\kappa$ values have drift rates dominated by the diurnal Yarkovsky effect, rather than the seasonal effect and thus have faster drift rates. This was done to establish an lower limit on the delivery timescales for the smaller Juno family members. Future models can more completely explore other $\kappa$ values that may better represent S-type asteroids.  

 Separately, those particles would be arriving into Earth-crossing orbits $\sim$ 275 Myr ago and are not likely to be easily accessible in the meteoritic record. Unlike with the L chondrites no such fossil meteorites have been found. If Juno is indeed responsible for 50\% of H chondrites than several conditions must be true:
\begin{enumerate}
    \item A smaller Juno family member, or members, $\geq$ 1km  in size experienced a breakup event 7-8 Myr ago while drifting inbound, at a semi-major axis of approximately 2.56 AU. This location is well within the total drift expected for 1 km asteroids over 300 Myr originating from the Juno family forming event (c.f Fig \ref{fig:scatter_props}).
    \item 1 meter asteroids resulting from this breakup would be able to reach the 3:1 resonance within 6 Myr assuming the Yarkovsky force drift rates described in Table \ref{tab:init_parameters}. The cosmic ray exposure age begins at the formation of objects $\leq$3 meters in size, so these particles begin with an effective CRE age of 0 at the breakup.
    \item Assuming the mean lifetimes and probabilities of orbits entering the 3:1 resonance and Earth-crossing orbits of \cite{morbidelli2002origin} a significant number of small asteroids would arrive in Earth-crossing orbits 7-8 Myrs after the breakup event, explaining both a shock degassing age of 300 Myr and a CRE age of 8 Myr. 
\end{enumerate}

With this conclusion comes a bit of nuance in the naming schemes that we must use when discussing meteorite parent bodies. In the situation presented above, where Juno is the original source of H chondrite meteorites, a two-step process is needed to adequately explain the paleomagnetic, shock degassing, and cosmic ray exposure age evidence of a large fraction of H chondrites. Throughout this paper we refer to the parent body of the initial family as the parent body of the H chondrite family. We adopt the term "secondary body" to refer to the Juno family member that would have broken up to supply the the spike of H chondrites with cosmic ray exposure ages with 7-8 Myrs. 

This solution is also in agreement with a few first-order approximations. Ordinary chondrite accumulation on the Earth is estimated to be 2900 - 7300 kg/yr \citep{bland1996flux}. Given that the 34\% of chondrites are H chondrites we will use the upper limit of 7300 kg/yr to find that approximately 2482 kg/yr of are are H chondrites. Given that approximately 50\% of these H chondrites exhibit the relevant CRE and shock degassing ages and assuming a 50\% ablation of mass during atmospheric re-entry, which will then cancel, we can estimate the total pre-atmospheric mass of H chondrites relevant to our parent body. Over the halflife of asteroids in Earth-crossing orbits from the 3:1 resonance found in \cite{1997Sci...277..197G}, 2.2 Myrs, this total mass is approximately 10$^{10}$ kg. This is just 0.7\% of the total mass entering the 3:1 resonance, according to \cite{1997Sci...277..197G}, leading to an initial asteroid mass of 1.4$\times$10$^{12}$ kg.  Assuming a bulk density for H chondrites of 3500 kg/m$^{3}$ we can then find that total volume, and thus radius, of the secondary body. We find the total initial volume is 4$\times$10$^{9}$ m$^{3}$ and a radius of 997 meters. This places the secondary body's size slightly above the modeled 1 kilometer diameter in the simulation but capable of reaching the necessary 2.56 au mark within 300 million years.

This tiered scale is also in agreement with the modeled collisional lifetime of km-sized asteroids in the main-belt from \citet{bottke_linking_2005}. Using both dynamical and collisional models of the main belt \citet{bottke_linking_2005} showed that asteroids with diameters of $\sim$1 km have collisional lifetimes of approximately 200 Myrs, similar to the results of \citet{farinella_meteorite_1998}. 

If such a secondary family exists and has typical S-type albedos it could be observable by the Vera Rubin Observatory, formerly known as the Large Synoptic Survey Telescope (LSST.) The current estimate for main belt asteroids is detections down to 100 meter in size, which may be enough to capture some of the larger fragments of the hypothesized secondary family \citep{the_lsst_solar_system_science_collaboration_solar_2009}. These larger fragments will not have experienced substantial Yarkovksy drift in the 7-8 Myr since the family forming event. However, given the relatively small size of the colliding objects, approximately 1000 and 500 meters in radius, respectively, relatively few $\sim$100 meter fragments should result. Confirming the spectral type of such objects becomes even more difficult. There is no near-infrared telescope capable of obtaining adequate signal-to-noise ratios for spectra of objects with an H magnitude around 22 as of the publication of this paper. A quick investigation using the Large Binocular Telescope exposure time calculator\footnote{http://luci-etc.lbto.org/calculator.py} confirms that an excessive amount of time would need to be allocated in order to obtain an SNR of 10. 

 To first order we can calculate the asteroid spatial distribution required to disrupt a one kilometer size body about once every few hundred million years with the following equation from \cite{2002aste.book..545D}. 
\begin{equation}
    N_{coll}=P_i(r_{impactor}+r_{target})^{2} N_{obj} T
\end{equation}
where, P$_i$ is the collisional frequency per area (yr$^{-1}$ km$^{-2}$), r$_{impactor}$ and r$_{target}$ are the radii of the colliding asteroids, , V is the relative velocity between the two asteroids, and N$_{obj}$ is the spatial density of asteroids in intersecting orbits with the target that match the required radius to disrupt the target, and T is time in years. Rearranging to find N$_{obj}$, setting N$_{coll}$ equal to 1, and implementing P$_i$=2.85$\times$10$^{-18}$ yr$^{-1}$km$^{-2}$ for V=5.81 km s${-1}$ from \cite{2002aste.book..545D}, with r$_{impactor}$ and r$_{target}$ of 300 and 1000 meters, with T of 300 Myrs, we find
\begin{equation}
    N_{obj} = \frac{1}{P_i (r_{impactor}+r_{target})^{2} T} = 6.9\times10^{8} 
\end{equation}
or approximately 700 million asteroids both capable of disrupting a $\sim$1 km Juno family member and with orbits that cross that of the hypothetical member, with roughly 73\% the mass of Vesta between all of them. Given the frequency of interaction with other Juno family members and their likelihood of collision we stress that this is an upper limit estimate for N$_{obj}$. 
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{one_meter_a_e.pdf}
    \caption{Eccentricity vs. semi-major axis for the 1000 modeled 1 meter test particles over the duration of the simulation. Notice that all particles are effectively removed by 80 Myrs. Interaction boundaries with Mars and Jupiter (semi-major axis + 3$\times$ R$_{Hill}$) are plotted in orange and blue, respectively. Significant resonances with Jupiter ( the 3:1, 8:3, and 5:2, left to right) are plotted with vertical lines.  Inward drifting particles are efficiently scattered by the 3:1 resonance with Jupiter but a large fraction of outward drifting particles make it all the way to the 2:1 resonance with Jupiter before scattering.}  
    \label{fig:a_e_t}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{one_m_particle_history.pdf}
    \caption{Overlaid particle histories for $a$,$e$,and $i$ for one-meter particles. Vertical lines represent scattering events that result in the removal of the particle from the simulation. Darker color represents a higher density of particles with similar properties, lighter colors indicates a lower density.}
    \label{fig:particle_history}
\end{figure*}
\begin{figure*}
\begin{tabular}{c c}
     \includegraphics[width=0.5\linewidth]{scattered_particles_1m.png} & \includegraphics[width=0.5\linewidth]{scattered_particles_10m.png}  \\
     (a) 1 meter &  (b) 10 meters \\
     \includegraphics[width=0.5\linewidth]{scattered_particles_100m.png} & \includegraphics[width=0.5\linewidth]{scattered_particles_1km.png}  \\
     (c) 100 meters &  (d) 1 kilometer  \\
\end{tabular} 
\label{fig:scatter_props}
\caption{Last reported a vs. e prior to scattering for each test particle size. Notice that for the smaller (1-10 meter) modeled particles that the J3:1 and 5:2 resonances are the major sources of scattering at 2.5 and 2.82 au, respectively. For the 100 modeled particles the long residency time within the J8:3 begins to become important as well, producing a more uniform distribution in e vs a space. For the 1 km particles, which do not reach the J3:1 or 5:2, the 8:3 is the main source of scattering due to the proximity to Juno and the long residency times, due to the particle's low drift rate. }
\end{figure*}
\begin{figure*}
\begin{tabular}{c c}
     \includegraphics[width=0.5\linewidth]{semimajor_ejection_histogram.png} & \includegraphics[width=0.5\linewidth]{time_ejection_histogram.png}  \\
     (a) &  (b)  \\
     \includegraphics[width=0.5\linewidth]{eccentricity_ejection_histogram.png} & \includegraphics[width=0.5\linewidth]{inclination_ejection_histogram.png}  \\
     (c)  &  (d)\\
\end{tabular} 
\label{fig:histograms}
\caption{ Histograms detailing times and orbital parameters that particles reached interactions with Mars or Jupiter. Note that large spikes in a) indicate the J3:1 and 5:2 resonances, while in b) they are representative of the time at which particles arrive at those those same resonances. In particular note the flat distribution for the 1 km partilcles. Figures c) and d) show no particularly strong dependence on eccentricity or inclination for the scattering particles.}
\end{figure*}

We recognize that this two-step solution is not necessarily unique to Juno and that investigations of other potential candidates with a similar experiment are critical to eliminate other potential candidates like (6) Hebe. We hope to expand and refine this method of dynamical modeling for these future attempts. 
